A Robust Specification Theory for Modal Event-Clock Automata

In a series of recent work, we have introduced a general framework for quantitative reasoning in specification theories. The contribution of this paper is to show how this framework can be applied to yield a robust specification theory for timed specifications.

==> eptcsdata.tex <==
\providecommand{\firstpage}{5}
\providecommand{\publicationstatus}{S. Bauer, J.-B. Raclet (Eds.): 4th International Workshop\\ on Foundations of Interface Technologies (FIT 2012)\\
EPTCS 87, 2012, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.87.2}{10.4204/EPTCS.87.2}}

